Efficient Parallel Self-Assembly Under Uniform Control Inputs

We prove that by successively combining subassemblies, we can achieve sublinear construction times for "staged" assembly of micro-scale objects from a large number of tiny particles, for vast classes of shapes; this is a significant advance in the context of programmable matter and self-assembly for building high-yield micro-factories.The underlying model has particles moving under the influence of uniform external forces until they hit an obstacle; particles bond when forced together with a compatible particle. Previous work considered sequential composition of objects, resulting in construction time that is linear in the number N of particles, which is inefficient for large N. Our progress implies critical speedup for constructible shapes; for convex polyominoes, even a constant construction time is possible. We also show that our construction process can be used for pipelining, resulting in an amortized constant production time.

==> 05-production.tex <==
\section{Production Problem is NP-hard}

\begin{theorem}
	The production problem, if a specific polyomino can be constructed in a given labyrinth, is NP-hard.
\end{theorem}

\begin{proof}
	Idea: Reduce from 3SAT in a similar fashion like in the hardness proof for \textsc{GlobalControl-ManyParticles} in \emph{Reconfiguring Massive Particle Swarms with Limited, Global Control}.
	Assign color red to every odd clause and blue to every even clause, i.e., there are only tiles of one type per clause. If a clause is satisfiable, one of the three will pass to the next step.
	If all clauses are satisfied, then we can build a line of length $|C|$ and flush it out of the labyrinth.
	Therefore:
	If and only if the 3SAT instance is satisfiable, we can produce a line with $|C|$ tiles. 
\end{proof}
